From if to Oops: Turning a conditional into a key-recovery oracle

Deterministic variants of CSIDH remove randomness from the group action, either through implementation techniques or, as in Houben's deterministic CSIDH and OSIDH-LD, by design. Since earlier fault attacks on CSIDH mostly target random point sampling, determinism seems to close that avenue. We show that it opens another: every secret-dependent step occurs at a fixed, public point of every execution, so an attacker can fault the same step repeatedly. Our attack forces the mask that selects which of two lanes computes the next isogeny to zero, for example by skipping one instruction. Whether the output changes reveals whether a secret exponent reaches a chosen threshold, and a binary search over these thresholds recovers the full key with one fault per execution: at most 297 oracle queries for OSIDH-LD and 222 for deterministic CSIDH with CSIDH-512-sized keys. We recover full OSIDH-LD keys in a software fault simulation of the reference implementation, and show on a ChipWhisperer-Lite that the targeted instruction is skipped with probability at least 0.94 at an isolated fault position. Finally, we argue that fault resistance requires giving up determinism, and propose countermeasures relying on randomization.

==> app_code.tex <==
\fixme{add the differences between alg 3 from Marc and C code}

==> app_osidh.tex <==
The fault site identification, software proof of concept, and idealized
recovery oracle for OSIDH-LD are presented in
\Cref{sec:osidh,sec:attack:osidh,sec:results:osidh} of the main body.
This appendix collects three structural features of the OSIDH-LD
implementation that may make practical faulting easier than in the
deterministic CSIDH setting, and that we leave as directions for future
experimental work.

\subsection{Potential amplification factors}

\paragraph{Cycle dimension.}
The outer loop repeats the same secret-dependent threshold test across
all $r = 13$ orientation tuples in each iteration. This provides
multiple glitch opportunities per execution where the same secret
component is used in the same logical role, and all of them return the
same oracle bit, so the attacker does not need to resolve which one a
glitch lands on. Under the single-fault model of
\Cref{sec:attack:model} this relaxes the timing precision required
rather than raising the per-execution success probability. We view this
as a useful engineering intuition rather than a proved attack
complexity.

\paragraph{AVX-512 lanes.}
The vectorised implementation in \texttt{protocols/avx512ifma/}
preserves the same masked lane-selection pattern in AVX-512 registers.
A low-level fault on the vectorised path may therefore affect several
orientation tuples simultaneously, potentially amortising the per-query
fault cost across the cycle. Quantifying this effect requires a
separate instruction-level study.

\paragraph{Public strategy order.}
The strategy-based variant (\texttt{eval\_action\_stra}) processes
primes in a fixed order determined at compile time. This makes timing
alignment strictly easier for the attacker than in non-deterministic
schemes, because the logical event $(u,i,t)$ is tied to a reproducible
point in each execution---the same property exploited in the
deterministic CSIDH setting.

%\subsection{Takeaway}

%Together, these factors suggest that hardware glitching against OSIDH-LD
%would face a lower practical barrier than the raw query count of $297$
%implies, chiefly by easing the trigger isolation identified in
%\Cref{sec:results:osidh-chip} as the remaining step. 

==> conclusion.tex <==
TODO


==> settings.tches.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2569-2925}
\makeatletter
\setDOI{10.46586/tches.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother

\setkeys{IACR}{journal=tches}


==> settings.tosc.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2519-173X}
\makeatletter
\setDOI{10.46586/tosc.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother

